Thresholding at the monopoly price: an agnostic way to improve bidding strategies in revenue-maximizing auctions

We address the problem of improving bidders' strategies in prior-dependent revenue-maximizing auctions and introduce a simple and generic method to design novel bidding strategies if the seller uses past bids to optimize her mechanism. We propose a simple and agnostic strategy, independent of the distribution of the competition, that is robust to mechanism changes and local (as opposed to global) optimization of e.g. reserve prices by the seller. This strategy guarantees an increase in utility compared to the truthful strategy for any distribution of the competition. In textbook-style examples, for instance with uniform [0,1] value distributions and two bidders, this no-side-information and mechanism-independent strategy yields an enormous 57% increase in buyer utility for lazy second price auctions with monopoly reserves. When the bidder knows the distribution of the highest bid of the competition, we show how to optimize the tradeoff between reducing the reserve price and beating the competition. Our formulation enables to study some important robustness properties of the strategies, showing their impact even when the seller is using a data-driven approach to set the reserve prices. In this sample-size setting, we prove under what conditions, thresholding bidding strategies can still improve the buyer's utility. The gist of our approach is to see optimal auctions in practice as a Stackelberg game where the buyer is the leader, as he is the first one to move (here bid) when the seller is the follower as she has no prior information on the bidder.

==> figures/ProofsSec3Thresholding.tex <==
%!TEX root = main.tex
\begin{proof}[Proof of Theorem thm:2StepProcessCommitment]
Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price. 

Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through. 
\end{proof}

\begin{lemma}[Phase transition]\label{app:lemma:phaseTransition}
Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases. 

Then there is a critical value $\alpha_c$ for which, if $\alpha<\alpha_c$, it is preferable for the bidder to threshold and if $\alpha>\alpha_c$, it is preferable for the bidder to bid truthfully. 	
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:phaseTransition}]
When $G_1=G_2=G$, we have ${\mathcal G}_\alpha=G$. Hence $U(r)$ does not depend on $\alpha$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\alpha$; let us call it $U^*(G)$.

On the other hand, we have 
$$
U(0)=\alpha\Exp{(X-\psi(X))G(X)}+(1-\alpha)\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
$$
Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0)$ is increasing in $\alpha$. In the rest of the proof we denote $U(0)$ by $U(0;\alpha)$ to stress its dependence on $\alpha$. 

The results for $\alpha=0$ correspond to \cite{nedelec2018thresholding}.  So we know that as $\alpha\tendsto 0$ $U(0;\alpha)<U^*(G)$. Indeed, thresholding at the monopoly price $r=\psi^{-1}(0)$ beats bidding truthful in that case. And optimal thresholding beats thresholding at the monopoly price.  On the other hand, $U(0;\alpha=1)>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\alpha)$ is an increasing function of $\alpha$, and is obviously continuous, we see that there exists a unique $\alpha_c$ such that if $\alpha<\alpha_c$, it is preferable for the buyer to shade her bid and above it, it is preferable to bid truthful. 

\nek{probably needs $\psi^{-1}(0)\neq 0$ somewhere}

\end{proof}
%
% We suppose in this subsection that the seller commits to thresholding. We note that when $r\geq \psi^{-1}(0)$,
% We have the following theorem.
% \begin{theorem}\label{thm:2StepProcessCommitment}
% We call ${\mathcal G}_\gamma=G_1+\gamma G_2$.
% If the buyer uses a $(r,0)$-thresholding strategy and commits to it, we have for their utility, if the seller is welfare benevolent~:
% if $r\geq \psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X{\mathcal G}_\gamma\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X)){\mathcal G}_\gamma(X)\indicator{X\geq r}}\;.
% \end{equation}
% if $r<\psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X G_1\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X))\left[G_1(X)\indicator{X\geq r}+\gamma G_2(X)\indicator{X\geq \psi^{-1}(0)}\right]}\;.
% \end{equation}
%
% This utility has a discontinuity at $r=\psi^{-1}(0)$. For $r<\psi^{-1}(0)$, we have $U(0)\geq U(r)$. For $r>\psi^{-1}(0)$, the first order condition are the same as in \nek{cite our work} where the distribution of the competition is now ${\mathcal G}_\gamma=G_1+\gamma G_2$. Call $r^*(\gamma)$ the unique solution to this problem.
%
% Hence, the optimal threshold is $\argmax_{r\in \{0,r^*_\gamma\}} U(r)$. When the optimal threshold is 0, our bid is truthful, of course.
%
% \end{theorem}
% \begin{proof}
% Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price.
%
% Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through.
% \end{proof}
%
% \begin{lemma}[Phase transition]\label{lemma:phaseTransition}
% Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases.
%
% Then there is a critical value $\gamma_c$ for which, if $\gamma>\gamma_c$, it is preferable for the bidder to threshold and if $\gamma<\gamma_c$, it is preferable for the bidder to bid truthfully.
% \end{lemma}
%
% \begin{proof}
% When $G_1=G_2=G$, we have ${\mathcal G}_\gamma/(1+\gamma)=G$. Hence $U(r)/(1+\gamma)$ does not depend on $\gamma$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\gamma$; let us call it $U^*(G)$.
%
% On the other hand, we have
% $$
% \frac{U(0;\gamma)}{1+\gamma}=\frac{1}{1+\gamma}\Exp{(X-\psi(X))G(X)}+\frac{\gamma}{1+\gamma}\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
% $$
% Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0;\gamma)/(1+\gamma)$ is decreasing in $\gamma$.
%
% The results for $\gamma=\infty$ correspond to \nek{cite our papers.}  So we know that as $\gamma\tendsto \infty$ $U(0;\gamma)/(1+\gamma)<U^*(G)$. On the other hand, $U(0;\gamma=0)/1>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\gamma)/(1+\gamma)$ is a decreasing function, and is obviously continuous, we see that there exists a unique $\gamma_c$ such that if $\gamma>\gamma_c$, it is preferable for the buyer to shade her bid and below it, it is preferable to bid truthful.
%
% \end{proof}

% \subsection{Existence of a Nash equilibrium in the two-stage game}
% Our approach here is the following. All players have essentially two strategies, according to Theorem \ref{thm}. They can either threshold optimally above the monopoly price or bid truthfully. We consider the first order conditions for a Nash equilibrium if all players threshold and we then study the best response of the remaining player.
%
% \begin{theorem}
% We consider the symmetric case and assume that the value distribution of the buyer is regular and follows the assumption of Theorem \ref{thm:nashEquiThresholded}.
% There exists $\alpha_{c,\text{thresh}}$ (possibly 0 or $\infty$) such that if $\alpha\leq \alpha_{c,\text{tresh}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies. It is the same as in the case $\alpha=0$ and the revenue of the bidders is the same as in a second price auction with no reserve.
%
% There exists $\alpha_{c,\text{truthful}}$ (possibly 0 or $\infty$) such that if $\alpha\geq \alpha_{c,\text{truthful}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies and it corresponds to bidding truthfully.
% \end{theorem}
% We provide more precise characterizations of the critical $\alpha$'s in the Appendix \nek{say where}
\begin{proof}[Proof of Theorem \ref{thm:ExistenceNashEqui2Stage}]
It is clear that each buyer's best response is either to bid truthful or to threshold optimally in the class of strategies we consider. 	

The theorem follows from Lemma \ref{lemma:phaseTransition}.	\textbf{1) Part 1.} For the first part, we suppose that all players except 1 plays the optimal thresholded strategy characterized by $r^*$ the unique solution of the equation 
$$
\frac{K-1}{r(1-F(r))}\Exp{XF^{K-2}(X)(1-F(X))\indicator{X\leq r}}=F^{K-1}(r)\;.
$$
This gives rise to the competition distribution 
$$
G_\beta(x;r^*)=F^{K-1}(\beta^{-1}(x))=\left(1-\frac{r^*(1-F(r^*))}{x}\right)^{K-1}\indicator{r^*(1-F(r^*))\leq x \leq r^*}+F^{K-1}(x)\indicator{x\geq r^*}\;.
$$
According to Lemma \ref{lemma:phaseTransition}, for this distribution $G_\beta(x;r^*)$, there exists $\alpha_{c,\text{thresh}}$ such that if $\alpha<\alpha_{c,\text{thresh}}$, the best response of the buyer in the class we consider is to threshold at $r>\psi^{-1}(0)$. Our results on Nash equilibria \nek{put a reference} in the case $\alpha=0$ \nek{check case no exploration}. By construction the optimal $r$ for this buyer is $r^*$ and we have the Nash equilibrium. 

Of course, if $\alpha>\alpha_{c,\text{thresh}}$, the best response of the buyer is to bid truthfully and hence there cannot be a Nash equilibrium in thresholding above $\psi^{-1}(0)$. 

\textbf{2) Part 2.} If all the players except one bid truthfully, Lemma \ref{lemma:phaseTransition} applies with $G=F^{K-1}$ and says that there exists $\alpha_{c,\text{truthful}}$, such that if $\alpha>\alpha_{c,\text{truthful}}$ the best response of the last player is to bid truthful. Hence there is a Nash equilibrium in the class we consider. On the other hand, if $\alpha<\alpha_{c,\text{truthful}}$, the best response of the last player is to threshold above $\psi^{-1}(0)$ and hence there is no Nash equilibrium. 

	
\end{proof}


==> figures/ProofsSec3Thresholding_copie.tex <==
%!TEX root = main.tex
\begin{proof}[Proof of Theorem thm:2StepProcessCommitment]
Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price. 

Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through. 
\end{proof}

\begin{lemma}[Phase transition]\label{app:lemma:phaseTransition}
Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases. 

Then there is a critical value $\alpha_c$ for which, if $\alpha<\alpha_c$, it is preferable for the bidder to threshold and if $\alpha>\alpha_c$, it is preferable for the bidder to bid truthfully. 	
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:phaseTransition}]
When $G_1=G_2=G$, we have ${\mathcal G}_\alpha=G$. Hence $U(r)$ does not depend on $\alpha$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\alpha$; let us call it $U^*(G)$.

On the other hand, we have 
$$
U(0)=\alpha\Exp{(X-\psi(X))G(X)}+(1-\alpha)\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
$$
Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0)$ is increasing in $\alpha$. In the rest of the proof we denote $U(0)$ by $U(0;\alpha)$ to stress its dependence on $\alpha$. 

The results for $\alpha=0$ correspond to \cite{nedelec2018thresholding}.  So we know that as $\alpha\tendsto 0$ $U(0;\alpha)<U^*(G)$. Indeed, thresholding at the monopoly price $r=\psi^{-1}(0)$ beats bidding truthful in that case. And optimal thresholding beats thresholding at the monopoly price.  On the other hand, $U(0;\alpha=1)>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\alpha)$ is an increasing function of $\alpha$, and is obviously continuous, we see that there exists a unique $\alpha_c$ such that if $\alpha<\alpha_c$, it is preferable for the buyer to shade her bid and above it, it is preferable to bid truthful. 

\nek{probably needs $\psi^{-1}(0)\neq 0$ somewhere}

\end{proof}
%
% We suppose in this subsection that the seller commits to thresholding. We note that when $r\geq \psi^{-1}(0)$,
% We have the following theorem.
% \begin{theorem}\label{thm:2StepProcessCommitment}
% We call ${\mathcal G}_\gamma=G_1+\gamma G_2$.
% If the buyer uses a $(r,0)$-thresholding strategy and commits to it, we have for their utility, if the seller is welfare benevolent~:
% if $r\geq \psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X{\mathcal G}_\gamma\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X)){\mathcal G}_\gamma(X)\indicator{X\geq r}}\;.
% \end{equation}
% if $r<\psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X G_1\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X))\left[G_1(X)\indicator{X\geq r}+\gamma G_2(X)\indicator{X\geq \psi^{-1}(0)}\right]}\;.
% \end{equation}
%
% This utility has a discontinuity at $r=\psi^{-1}(0)$. For $r<\psi^{-1}(0)$, we have $U(0)\geq U(r)$. For $r>\psi^{-1}(0)$, the first order condition are the same as in \nek{cite our work} where the distribution of the competition is now ${\mathcal G}_\gamma=G_1+\gamma G_2$. Call $r^*(\gamma)$ the unique solution to this problem.
%
% Hence, the optimal threshold is $\argmax_{r\in \{0,r^*_\gamma\}} U(r)$. When the optimal threshold is 0, our bid is truthful, of course.
%
% \end{theorem}
% \begin{proof}
% Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price.
%
% Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through.
% \end{proof}
%
% \begin{lemma}[Phase transition]\label{lemma:phaseTransition}
% Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases.
%
% Then there is a critical value $\gamma_c$ for which, if $\gamma>\gamma_c$, it is preferable for the bidder to threshold and if $\gamma<\gamma_c$, it is preferable for the bidder to bid truthfully.
% \end{lemma}
%
% \begin{proof}
% When $G_1=G_2=G$, we have ${\mathcal G}_\gamma/(1+\gamma)=G$. Hence $U(r)/(1+\gamma)$ does not depend on $\gamma$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\gamma$; let us call it $U^*(G)$.
%
% On the other hand, we have
% $$
% \frac{U(0;\gamma)}{1+\gamma}=\frac{1}{1+\gamma}\Exp{(X-\psi(X))G(X)}+\frac{\gamma}{1+\gamma}\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
% $$
% Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0;\gamma)/(1+\gamma)$ is decreasing in $\gamma$.
%
% The results for $\gamma=\infty$ correspond to \nek{cite our papers.}  So we know that as $\gamma\tendsto \infty$ $U(0;\gamma)/(1+\gamma)<U^*(G)$. On the other hand, $U(0;\gamma=0)/1>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\gamma)/(1+\gamma)$ is a decreasing function, and is obviously continuous, we see that there exists a unique $\gamma_c$ such that if $\gamma>\gamma_c$, it is preferable for the buyer to shade her bid and below it, it is preferable to bid truthful.
%
% \end{proof}

% \subsection{Existence of a Nash equilibrium in the two-stage game}
% Our approach here is the following. All players have essentially two strategies, according to Theorem \ref{thm}. They can either threshold optimally above the monopoly price or bid truthfully. We consider the first order conditions for a Nash equilibrium if all players threshold and we then study the best response of the remaining player.
%
% \begin{theorem}
% We consider the symmetric case and assume that the value distribution of the buyer is regular and follows the assumption of Theorem \ref{thm:nashEquiThresholded}.
% There exists $\alpha_{c,\text{thresh}}$ (possibly 0 or $\infty$) such that if $\alpha\leq \alpha_{c,\text{tresh}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies. It is the same as in the case $\alpha=0$ and the revenue of the bidders is the same as in a second price auction with no reserve.
%
% There exists $\alpha_{c,\text{truthful}}$ (possibly 0 or $\infty$) such that if $\alpha\geq \alpha_{c,\text{truthful}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies and it corresponds to bidding truthfully.
% \end{theorem}
% We provide more precise characterizations of the critical $\alpha$'s in the Appendix \nek{say where}
\begin{proof}[Proof of Theorem \ref{thm:ExistenceNashEqui2Stage}]
It is clear that each buyer's best response is either to bid truthful or to threshold optimally in the class of strategies we consider. 	

The theorem follows from Lemma \ref{lemma:phaseTransition}.	\textbf{1) Part 1.} For the first part, we suppose that all players except 1 plays the optimal thresholded strategy characterized by $r^*$ the unique solution of the equation 
$$
\frac{K-1}{r(1-F(r))}\Exp{XF^{K-2}(X)(1-F(X))\indicator{X\leq r}}=F^{K-1}(r)\;.
$$
This gives rise to the competition distribution 
$$
G_\beta(x;r^*)=F^{K-1}(\beta^{-1}(x))=\left(1-\frac{r^*(1-F(r^*))}{x}\right)^{K-1}\indicator{r^*(1-F(r^*))\leq x \leq r^*}+F^{K-1}(x)\indicator{x\geq r^*}\;.
$$
According to Lemma \ref{lemma:phaseTransition}, for this distribution $G_\beta(x;r^*)$, there exists $\alpha_{c,\text{thresh}}$ such that if $\alpha<\alpha_{c,\text{thresh}}$, the best response of the buyer in the class we consider is to threshold at $r>\psi^{-1}(0)$. Our results on Nash equilibria \nek{put a reference} in the case $\alpha=0$ \nek{check case no exploration}. By construction the optimal $r$ for this buyer is $r^*$ and we have the Nash equilibrium. 

Of course, if $\alpha>\alpha_{c,\text{thresh}}$, the best response of the buyer is to bid truthfully and hence there cannot be a Nash equilibrium in thresholding above $\psi^{-1}(0)$. 

\textbf{2) Part 2.} If all the players except one bid truthfully, Lemma \ref{lemma:phaseTransition} applies with $G=F^{K-1}$ and says that there exists $\alpha_{c,\text{truthful}}$, such that if $\alpha>\alpha_{c,\text{truthful}}$ the best response of the last player is to bid truthful. Hence there is a Nash equilibrium in the class we consider. On the other hand, if $\alpha<\alpha_{c,\text{truthful}}$, the best response of the last player is to threshold above $\psi^{-1}(0)$ and hence there is no Nash equilibrium. 

	
\end{proof}


==> two_stage_subsection.tex <==
Recent work have shown the seller can implement strategies to prevent or limit the possibility for bidders to be strategic \citep{amin2013learning, mohri2015revenue, golrezaei2018dynamic}. In the case of an infinitely patient seller (against a finitely patient bidder), the explore-exploit strategies proposed, based on alternance between exploration and exploitation, can force bidders to be (almost) truthful and ensure the possibility to maximize the revenue by estimating and using the empirical monopoly price. \citet{amin2013learning} also highlights that when the seller is not infinitely patient, the value has to be shared between the seller and the bidders. Hence, it is important for us to study how our strategy is robust to such exploration / exploitation mechanism on the seller side and how the value is shared between both when neither seller or bidders are infinitely patients.

We consider the two-step mechanism as proposed in \cite{amin2013learning, golrezaei2018dynamic} that can be described as a tuple of the form $P= (G, H, r, F)$ that is defined as follows: 
\begin{description}
\item[1 -- exploration] The seller runs a lazy 2$^\text{nd}$-price auction. The current bidder faces a competition $G$. In this step, the randomized reserve price is formalized by the distribution $H$.
\item[2 -- exploitation] The seller runs a lazy 2$^\text{nd}$-price auction with reserve price $r$, possibly personalized. The current bidder faces the same competition $G$ as in the first step.
\end{description}

\paragraph{Seller's revenue maximization.} As described in the aforementioned papers, the seller uses the distributions of bids observed in the first period to optimize the reserve in the second period. As we have shown previously that our strategy can be made robust to sellers approximation error (subsection \ref{sec:empirical_estimation}), this error is neglictible from the point of view of bidder's optimization problem and, to simplify the analysis, we assume after observing the exploration phase, the seller gets to use $r^*_{\beta}$. To make the dependency on the bidder's strategy $\beta$ explicit, we use the notation $P^{\beta} = (G, H, r^*_{\beta}, F)$. Note we study here a single repetition of this mechanism, as the doubling trick proposed in these papers is an artifact to derive regret bounds for a seller that is infinitely patient.

\paragraph{Bidders are commiting to the same strategy in both phases.} As highlighted by \cite{golrezaei2018dynamic}, the exploration auctions from the first period may come from past random exploration. Thus, phases may not be easily idenfiable for the bidders. We then assume the bidders are commiting to the same strategy in both phases by lack of idenfiability\footnote{Note a very similar study can be carried out if the bidders are allowed to use different strategies in both phases, it would lead the bidders to be truthful in the second phase. This is practically unrealistic as they would reveal their true value distribution in the second phase, giving the incentive to the seller to ``lie'' about on which phase he is estimating the personalized reserves.}.

\paragraph{Utility of the strategic bidder.} In this framework, the objective of the bidder is to choose a strategy $\beta$ to maximize a weighted sum of her utility in both phases:
\begin{align}
U_\alpha(\beta) = \alpha U_1(\beta) + (1-\alpha) U_2(\beta)
\end{align}
where $U_i$ is the expected utility of the bidder in stage $i$. The $\alpha \in [0,1]$ quantifies how much each step weights in the bidders objective. For instance, given a seller using $\eta T$ exploration auctions and $(1-\eta)T$ exploitation ones and a bidder optimizing on a finite horizon of length $\gamma T$, then in the worst case $\alpha = \frac{\gamma - \eta}{\gamma}$. Note, we need to consider a worst case for $\alpha$ as the bidder cannot identify the phases. More precisely, $U_1$ is the expected utility of a lazy second price with random reserve and $U_2$ is the expected utility of a lazy second price with monopoly reserves corresponding to $F_B$.


\begin{figure}[tbp]
  \centering
  % \includegraphics[width=0.48\textwidth]{nips_stackelberg_games/figures/strategies.pdf}
  % \includegraphics[width=0.48\textwidth]{nips_stackelberg_games/figures/revenues.pdf}
  \includegraphics[width=0.31\textwidth]{figures/strategies.pdf}
  \includegraphics[width=0.31\textwidth]{figures/revenues.pdf}
    %\includegraphics[width=0.32\textwidth]{nips_stackelberg_games/figures/virtual_values.pdf}
  \caption{Left: illustration of strategies. Right: function optimized by the seller $b(1-F_{B}(b))$ depending on the strategy for values distribution $F$ being $\mathcal{U}(0,1)$. $R$ is set at 0.2, $x_1$ is set such that $x_1(1-F(x_1)) = R$ (right root) and $x_0 \simeq 0.27$ for $\dtbeta$.}
  \label{fig:optimal_revenues}
\end{figure}
\iffalse
\cite{tang2016manipulate, nedelec2018thresholding} exhibited strategies for the case where the bidders only optimize for the utility of the second phase, i.e. $\alpha=0$. However, in practice, sellers use an exploration stage to learn the value distribution. Taking care of this exploration phase is of great importance for the bidders since optimizing only the second stage can lead to large loss of utility during the first stage. 

In Section \ref{sec:two-stage-process}, we extend the approach of \cite{tang2016manipulate, nedelec2018thresholding} to the two-stage game showing that the strategies which are optimal when the bidder is only optimizing her utility in the second stage are suboptimal when she takes into consideration the exploration stage of the seller. We find in Section \ref{sec:welfareSharing} the optimal strategy in this framework and study the behavior of this strategy as a function of the length of the exploration stage. To study whether the strategies are robust to the presence of other strategic bidders in the game, we also prove the existence of a Nash equilibrium under certain conditions and we compute the utility of the bidders and the revenue of the seller at this Nash equilibrium when it exists. 

Unlike \cite{amin2013learning, golrezaei2018dynamic}, we consider the objective function of the bidders to be the expected utility of the two stages instead of the utility computed on a finite number of auctions. Indeed, as there exists a high number of repeated auctions, billions a day in the case of online advertising, optimizing directly the expected utility makes sense from a bidder's standpoint. We extend our results to finite sample sizes in Section \ref{sec:empirical_estimation}. We finally show the strategies are robust to an estimation of the bidders' competition in Section \ref{sec:robust_competition} and to a change of mechanism in Section \ref{sec:change_mechanism}. It shows their robustness to most of the difficulties bidders practically face and provides concrete solutions to solve these problems.


\section{Understanding the strategic reaction of the players}
\label{sec:two-stage-process}
In order to get a good understanding of how the welfare is shared between seller and bidders when $\alpha$ moves from $0$ to $1$, we need to study the strategies of the different players. First, on the seller's side, she chooses the distribution of reserve prices $H$ faced by the strategic bidder in the first phase. At this point, we assume the seller does not have any knowledge about the bidders (except the support of the value distribution). Hence, she mostly has two choices for $H$: either no reserve price or a uniform distribution \cite{amin2014repeated}. In the second stage, the seller is assumed welfare-benevolent, i.e. if she has the choice between two reserve prices equivalent in terms of payment, she chooses the lowest one. Hence, in the second stage, the seller chooses $r^*_\beta = \inf \argmax_r R_B(r)$. 


From a bidder's standpoint, \cite[Th. 6.2]{tang2016manipulate} exhibits the best response for the extreme case $\alpha = 0$. Unfortunately, this best response induces a complicated optimization problem for the seller: $R_{B}$ is non-convex with several local optima and the global optimum is reached at a discontinuity of $R_{B}$ (see Fig. \ref{fig:optimal_revenues}). This is especially problematic if sellers are known to optimize reserve prices conditionally on some available context using parametric models such as Deep Neural Networks \cite{dutting2017optimal} whose fit is optimized via first-order optimization and hence would regularly fail to find the global optimum. This is undesirable for the bidders: in any Stackelberg game, the leader's advantage comes from being able to predict the follower's strategy.

To address this issue, \cite{tang2016manipulate,nedelec2018thresholding} proposed a \emph{thresholding strategy} that is the best response in the restricted class of strategies that ensure $R_{B}$ to be concave as long as $R_{X}$ is so, when $\alpha = 0$.
\fi

 We show that the thresholded strategies can be extended to the two-stage process with a slight modification. The requirement is to ensure $R_{B_i}$ to be \emph{quasi-}concave as long as $R_{X}$ is so. Then, we have the following result.
\begin{theorem}
Given a two-step process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$ and such that $F$ is quasi-regular\footnote{We say a distribution is quasi-regular if the associated revenue curve $R_{X_i}$ is quasi-concave}, $\forall \alpha\in[0,1], \,\exists 0 \leq x_0 \leq x_1$ such that the best quasi-regular response (maximizing $U_\alpha(\beta)$ with $F_B$ regular) is 
\vspace{-0.5em}
\begin{align}\label{eq:defDoubleThresh}
\dtbeta(x)
=
\indicator{x \leq x_0}x
+
\indicator{x_0 < x \leq x_1}\frac{R}{1-F(x)}
+
\indicator{x > x_1}x
~~~~~\text{where}~~~~~ R = x_1 (1 - F(x_1))
\end{align}
Moreover, we have $x_1 = \sup \{x: x(1-F(x)) \geq R\}$ and $x_0 \leq \overline{x}_0 = \inf \{x: x(1-F(x)) \geq R\}$.
\label{dfn:thresholded_beta}
\end{theorem}
The proof is in Appendix \ref{ssec:best_quasi_regular_response}.
\iffalse
\begin{remark}
The thresholding strategy introduced in Definition \ref{definition_thresholded_strategies} is a special case of $\dtbeta$ in the case when $x_0 = 0$ and we will denote it $\tbeta$ for simplicity. As we will see in Section \ref{sec:optimal_strategies}, when $\alpha$ is small enough (but not 0 yet), $x_0 = 0$ is optimal. It thus makes sense to study both these strategies.
\end{remark}
\fi
\iffalse
This class of strategies solves the main drawback of the best response from \cite{tang2016manipulate}. If the value distribution $F_i$ is quasi-regular, then the bid distribution $F_{B}$ is also quasi-regular, offering a quasi-concave maximization problem (thus ``predictable" for the buyer) to the seller.
Figure \ref{fig:optimal_revenues} illustrates the different strategies as well as the corresponding optimization problems and the virtual values associated to the push-forward bid distributions. Understanding the strategic answer of the bidders helps avoiding worst-case scenario reasoning when studying the revenue of the sellers against strategic bidders. We now quantify precisely how the welfare is shared between strategic bidders and seller.
\fi


%The literature have only considered so far the 
%possible bidding strategies: 
%\begin{definition}[Thresholded bidding strategies]\cite{tang2016manipulate,nedelec2018thresholding}
%\label{dfn:thresholded_beta}
% A bidding strategy $\beta$ is called a thresholded bidding strategy if and only if there exists $r>0$ such that for all $x < r, h_{\beta}(x) = \psi_B(\beta(x)) = 0$. This family of functions can be parametrized with
%\begin{equation*}
%\beta_r^\gamma(x)=\frac{\gamma(r)(1-F(r))}{1-F(x)}\indicator{x< r}+\gamma(x)\indicator{x\geq r}\;,
%\end{equation*}
%with $r \in \mathbb{R}$ and $\gamma: \mathbb{R} \rightarrow \mathbb{R}$ strictly increasing.
%\end{definition}
%
%This class of continuous bidding strategies has two degrees of freedom : the threshold $r$ such that for all $x < r, h_{\beta}(x) = 0$ and the strategy $\gamma$ used beyond the threshold. We do not restrict the class of functions of $\gamma$ that can be used beyond the threshold. All the strategies defined in this class have the property to have a reserve value equal to zero, i.e. their reserve price is equal to their minimum bid, when the seller is welfare benevolent and the virtual value of $\gamma$ is positive beyond $r$. We show that there exists an optimal threshold $r$ for the strategic bidder that depends on the competition and that the optimal strategy to use for $x > r$ is to be truthful. The next lemma computes this optimal thresholded strategy by deriving a variant of Lemma \ref{lemma:directDerivativeRevenueSecondPriceAuction} in the class of thresholded strategies.
%
%thresholded strategies with a dirac \cite{tang2016manipulate}
%
%
%neural networks to learn the best response \cite{nedelec2019learning}
\iffalse
\section{Welfare sharing between seller and buyers}\label{sec:welfareSharing}

\fi
This section presents how the welfare is shared in the two-stage process with strategic bidders. 
\iffalse
First, we show how to numerically compute the best response and illustrate the variation of utility and payment with $\alpha$. After remarking and showing that the \emph{thresholded} strategy \cite{nedelec2018thresholding} is optimal for greater values of $\alpha$ than 0, we focus on this strategy and show the existence of a Nash equilibrium. It proves that even in the case of multiple strategic bidders, there exists strategies that enable bidders to take advantage of the learning stage of the seller.
\fi
\subsubsection{Welfare sharing with best quasi-regular response}
\begin{figure}[tbp]
  \centering
    \includegraphics[width=0.32\textwidth]{figures/welfare_no_reserve_1_with_sum_thomas_utility.pdf}
     \includegraphics[width=0.32\textwidth]{figures/welfare_no_reserve_1_with_sum_thomas_payment.pdf}
  \includegraphics[width=0.32\textwidth]{figures/optimal_thresholds_no_reserve.pdf}
  \caption{Welfare sharing with random reserve in stage 1: Left -- Utility of strategic bidder in the two-stage game as a function of $\alpha$. Middle -- Payment of strategic bidder in the two-stage game as a function of $\alpha$. The dotted lines corresponds to phase 1, the dashed ones to phase 2 and the plain line for the full game. The blue color is used for the bidder's utility and the red for her payment. The black color is used for the baseline of truthful bidding. Right: evolution of $x_0^*, x_1^*$ with $\alpha$.}
  \label{fig:welfare_vs_alpha}
\end{figure}
\label{sec:optimal_strategies}
We first show how to obtain numerically the best response $\dtbeta$ by solving the maximization problem of $U_\alpha$ restricted to the class of strategies described in Th. \ref{dfn:thresholded_beta}. This allows us to show how the bidder's utility and payment vary with $\alpha$.
\begin{theorem}
Given a two-stage process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$, the best response is of the form of $\tilde{\beta}_{x_0^*, x_1^*}$ and the utility $U_\alpha(\dtbeta)$ has the following derivatives:
\begin{align}
    \frac{\partial U_\alpha(\dtbeta\!)}{\partial x_0} \!=\! \alpha(1-F(x_0))G(x_0)H(x_0)
    -
    x_0 f(x_0) G_\alpha\!\!\left(\frac{x_1(1-F(x_1))}{(1-F(x_0))}\right)~~~~~~~~~~~\\
    \frac{\partial U_\alpha(\dtbeta\!)}{\partial x_1} 
    \!= \!
    f(x_1)\psi(x_1)
    \!\left(\!G_\alpha(x_1) - \lE_X\!\!\left(\!\indicator{x_0 \leq X \leq x_1}\frac{X}{(1-F(X))}g_\alpha\!\!\left(\!\frac{x_1(1-F(x_1))}{(1-F(X))}\!\right)\!\!\right)\!\!\right)
\end{align}
where $G_\alpha(x) = \alpha G(x)H(x) + (1-\alpha)G(x)$ and $\psi(x)=x-\frac{1-F(x)}{f(x)}$.
\label{thm:double_thresholded_derivatives}
\end{theorem}
The proof is in Appendix \ref{ssec:welfare_sharing_best_response}. We now use these results to compute numerically the best response in the following two-stage process: $P_1 = (G\!=\!U_{[0,1]}, H\!=\!0, r^*_{\tilde{\beta}_{x_0^*, x_1^*}}, F\!=\!U_{[0,1]})$ (uniformly distributed reserve in  stage 1)
   
\iffalse  
$P_2 = (G\!=\!U_{[0,1]}, H\!=\!1, r^*_{\tilde{\beta}_{x_0^*, x_1^*}}\!, F\!=\!U_{[0,1]})$ (no reserve in stage 1).
\fi

The results are presented in Fig. \ref{fig:welfare_vs_alpha}.
First, we recover the results from the literature corresponding to the extremes values of $\alpha$. For $\alpha = 1^-$, the payment and utility in the second stage are the ones of a 2$^\text{nd}$-price with monopoly price of value distribution. As $\alpha$ decreases, the total payment over the two stages quickly decreases (and utility increases) towards values that are even more favorable to the bidder than the ones of a 2$^\text{nd}$-price with no reserve price. 
\iffalse
This is consistent with the observations from \cite{nedelec2018thresholding} (case $\alpha=0$): if only one bidder is strategic, the payment of this strategic bidder can decrease even further than the one of a 2$^\text{nd}$-price with no reserve price. 
In Appendix \ref{ssec:plot_with_random_reserve}, we provide the same study with random reserve and show that the presence of exploration of the reserve prices in the first period (difference between left and right) does not impact much the payment/utility of the second period. It slightly decreases the advantage of the bidder, but not significantly.
\fi
Finally, we observe two regimes for $x_0^*$ (Fig. \ref{fig:welfare_vs_alpha}, right): for $\alpha < 0.8$ it is 0 and for $\alpha > 0.8$ it is the value that saturates the inequality constraint described by Th. \ref{dfn:thresholded_beta} between $x_0$ and $x_1$. This illustrates why we cannot only use first-order optimality condition: the optimal value is often reached on the edge of the feasible domain. We formalize this latter observation and shows that when $\alpha$ is small enough, the reserve value $x_0^*$ is exactly 0.
\begin{lemma}
Given a two-step process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$. If $\exists y \in [0,b], \forall x<y, \frac{G(x)H(x)}{f(x)} < x$ and $\frac{G(x)H(x)}{f(x)}$ is bounded on $[0,x^*]$ with $x^*=\inf\argmax_x R_X(x)$, then $\exists \alpha_0 > 0$ such that $\forall \alpha < \alpha_0$, 
\begin{align*}
(x^*_0,x^*_1) \in \argmax_{x_0, x_1}U_\alpha(\dtbeta) 
~~~ \Rightarrow ~~~ 
x_0^* = 0
\end{align*}
\label{thm:x0_to_0}
\end{lemma}
\vspace{-1em}
The proof can be found in Appendix \ref{ssec:welfare_sharing_best_response}.  $\frac{G(x)H(x)}{f(x)}$ being bounded on $[0,x^*]$ is satisfied if $F$ is MHR (monotonous hazard rate). $\frac{G(x)H(x)}{f(x)}<x$ is the key assumption. Intuitively, it can be interpreted as \emph{"if the bidder has enough mass under the competition, she can overbid at almost no cost on small values to decrease the reserve value to 0."}
This theorem shows that the \emph{thresholding} strategies are actually optimal for $\alpha$ small enough and not just for $\alpha = 0$.


==> two_stage_subsection_old.tex <==
\iffalse
As it is classical in auction theory \cite{krishna2009auction}, we assume the valuation of a bidder $v \in \mathbb{R}$ is drawn from a specific distribution $F$ (the distribution can be different from one bidder to the other);  a bidding strategy is a mapping $\beta$ from $\mathbb{R}_+$ into  $\mathbb{R}_+$ that provides the actual bid $B=\beta(v)$ when the value is $v$. As a consequence, the distribution of bids $F_{B}$ is  the push-forward of $F$ by $\beta$. We assume from now on that the support of $F$ is $[0, b) \subseteq [0, +\infty]$. If $b = +\infty$, we additionally assume that $F$ verifies $1-F(x) = o(x^{-1})$ to avoid problems with the definition of the optimal reserve price. Unless otherwise noted $F$ is assumed to be regular.

The seller has an estimate of the bidders' bid distribution, typically coming from access to past bids. Then, she uses an approximation of a revenue-maximizing auction based on her estimate of the bid distributions. We will consider that this is a lazy 2$^\text{nd}$-price auction \cite{paes2016field} whose reserve price is optimized to maximize the \emph{seller's revenue}. For the lazy 2$^\text{nd}$-price auction, the optimal reserve price happens to be the \emph{monopoly price} $r^*_{\beta}$ which maximizes the \emph{monopoly revenue} 
$$
R_{B}(r) = r(1-F_{B}(r))
$$ extracted by the seller on the current bidder. 
\fi
We finally generalize our approach to a general two-step process \cite{amin2013learning,cole2014sample}: 
\paragraph{General two-step process with commitment:} A general two-step process with commitment is a tuple of the form $P= (G, H,r, F)$ that is defined as follows: %\nek{should this be called two-step process with commitment (of the others)? In general, there could be $G_{i,1}$ and $G_{i,2}$, i.e difference competition distribution in the second stage}
\begin{description}
\item[1 -- exploration] The seller runs a lazy 2$^\text{nd}$-price auction. The current bidder faces a competition $G$. In this step, the potential randomized or deterministic reserve price is denoted by the distribution $H$.
\item[2 -- exploitation] The seller runs a lazy 2$^\text{nd}$-price auction with reserve price $r$, possibly personalized. The current bidder faces the same competition $G$ as in the first step.
\end{description}

To make explicit the dependency on the bidder's strategy $\beta$ on the design of the auction of the second step when optimizing the reserve price based on the observation of the first period, we use the notation $P^{\beta} = (G, H, r^*_{\beta}, F)$.
The tradeoff between exploration and exploitation from the seller standpoint was introduced in \citep{amin2013learning} and refined in \cite{mohri2015revenue, golrezaei2018dynamic}. They introduce a parameter $\alpha$, $0\leq \alpha<1$, to define this trade-off, assuming the ratio of length between the first and the second stage is equal to $\alpha/1-\alpha$. \cite{amin2013learning} proved that if bidders are non-discounted buyers, there must exist a good strategy for them in this mechanism, forcing the seller to suffer a regret linear in the number of auctions. We are interested in solving the Stackelberg game faced by bidders when they know the seller is using this classical mechanism to learn their value distribution. Bidders are the leaders in this framework since they know the mechanism used by the seller and can choose their strategy accordingly.

We assume that the strategic bidder commits to the same strategy $\beta$ (inducing the same distribution of bids $F_{B}$) in both phases. This assumption accounts for the fact that in practice sellers regularly update their priors based on recent past bids, forcing the bidders to commit in the long-term to the bid distribution they want the seller to use as prior. Otherwise, the seller might discover new aspects of the buyer's bid distribution and change their mechanism accordingly more than once as time evolves.

In this framework, the objective of the bidder is to choose a strategy $\beta$ to maximize a weighted sum of her utility in both phases:
\begin{align}
U_\alpha(\beta) = \alpha U_1(\beta) + (1-\alpha) U_2(\beta)
\end{align}
where $U_i$ is the expected utility of the bidder in stage $i$. The $\alpha \in [0,1]$ quantifies the length of each stage \citep{amin2013learning}. More precisely, $U_1$ is the expected utility of a lazy second price without reserve/with random reserve and $U_2$ is the expected utility of a lazy second price with monopoly reserves corresponding to $F_B$.


\begin{figure}[tbp]
  \centering
  % \includegraphics[width=0.48\textwidth]{nips_stackelberg_games/figures/strategies.pdf}
  % \includegraphics[width=0.48\textwidth]{nips_stackelberg_games/figures/revenues.pdf}
  \includegraphics[width=0.31\textwidth]{figures/strategies.pdf}
  \includegraphics[width=0.31\textwidth]{figures/revenues.pdf}
    %\includegraphics[width=0.32\textwidth]{nips_stackelberg_games/figures/virtual_values.pdf}
  \caption{Left: illustration of strategies. Right: function optimized by the seller $b(1-F_{B}(b))$ depending on the strategy for values distribution $F$ being $\mathcal{U}(0,1)$. $R$ is set at 0.2, $x_1$ is set such that $x_1(1-F(x_1)) = R$ (right root) and $x_0 \simeq 0.27$ for $\dtbeta$.}
  \label{fig:optimal_revenues}
\end{figure}
\iffalse
\cite{tang2016manipulate, nedelec2018thresholding} exhibited strategies for the case where the bidders only optimize for the utility of the second phase, i.e. $\alpha=0$. However, in practice, sellers use an exploration stage to learn the value distribution. Taking care of this exploration phase is of great importance for the bidders since optimizing only the second stage can lead to large loss of utility during the first stage. 

In Section \ref{sec:two-stage-process}, we extend the approach of \cite{tang2016manipulate, nedelec2018thresholding} to the two-stage game showing that the strategies which are optimal when the bidder is only optimizing her utility in the second stage are suboptimal when she takes into consideration the exploration stage of the seller. We find in Section \ref{sec:welfareSharing} the optimal strategy in this framework and study the behavior of this strategy as a function of the length of the exploration stage. To study whether the strategies are robust to the presence of other strategic bidders in the game, we also prove the existence of a Nash equilibrium under certain conditions and we compute the utility of the bidders and the revenue of the seller at this Nash equilibrium when it exists. 

Unlike \cite{amin2013learning, golrezaei2018dynamic}, we consider the objective function of the bidders to be the expected utility of the two stages instead of the utility computed on a finite number of auctions. Indeed, as there exists a high number of repeated auctions, billions a day in the case of online advertising, optimizing directly the expected utility makes sense from a bidder's standpoint. We extend our results to finite sample sizes in Section \ref{sec:empirical_estimation}. We finally show the strategies are robust to an estimation of the bidders' competition in Section \ref{sec:robust_competition} and to a change of mechanism in Section \ref{sec:change_mechanism}. It shows their robustness to most of the difficulties bidders practically face and provides concrete solutions to solve these problems.


\section{Understanding the strategic reaction of the players}
\label{sec:two-stage-process}
In order to get a good understanding of how the welfare is shared between seller and bidders when $\alpha$ moves from $0$ to $1$, we need to study the strategies of the different players. First, on the seller's side, she chooses the distribution of reserve prices $H$ faced by the strategic bidder in the first phase. At this point, we assume the seller does not have any knowledge about the bidders (except the support of the value distribution). Hence, she mostly has two choices for $H$: either no reserve price or a uniform distribution \cite{amin2014repeated}. In the second stage, the seller is assumed welfare-benevolent, i.e. if she has the choice between two reserve prices equivalent in terms of payment, she chooses the lowest one. Hence, in the second stage, the seller chooses $r^*_\beta = \inf \argmax_r R_B(r)$. 


From a bidder's standpoint, \cite[Th. 6.2]{tang2016manipulate} exhibits the best response for the extreme case $\alpha = 0$. Unfortunately, this best response induces a complicated optimization problem for the seller: $R_{B}$ is non-convex with several local optima and the global optimum is reached at a discontinuity of $R_{B}$ (see Fig. \ref{fig:optimal_revenues}). This is especially problematic if sellers are known to optimize reserve prices conditionally on some available context using parametric models such as Deep Neural Networks \cite{dutting2017optimal} whose fit is optimized via first-order optimization and hence would regularly fail to find the global optimum. This is undesirable for the bidders: in any Stackelberg game, the leader's advantage comes from being able to predict the follower's strategy.

To address this issue, \cite{tang2016manipulate,nedelec2018thresholding} proposed a \emph{thresholding strategy} that is the best response in the restricted class of strategies that ensure $R_{B}$ to be concave as long as $R_{X}$ is so, when $\alpha = 0$.
\fi

 We show that the thresholded strategies can be extended to the two-stage process with a slight modification. The requirement is to ensure $R_{B_i}$ to be \emph{quasi-}concave as long as $R_{X}$ is so. Then, we have the following result.
\begin{theorem}
Given a two-step process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$ and such that $F$ is quasi-regular\footnote{We say a distribution is quasi-regular if the associated revenue curve $R_{X_i}$ is quasi-concave}, $\forall \alpha\in[0,1], \,\exists 0 \leq x_0 \leq x_1$ such that the best quasi-regular response (maximizing $U_\alpha(\beta)$ with $F_B$ regular) is 
\vspace{-0.5em}
\begin{align}\label{eq:defDoubleThresh}
\dtbeta(x)
=
\indicator{x \leq x_0}x
+
\indicator{x_0 < x \leq x_1}\frac{R}{1-F(x)}
+
\indicator{x > x_1}x
~~~~~\text{where}~~~~~ R = x_1 (1 - F(x_1))
\end{align}
Moreover, we have $x_1 = \sup \{x: x(1-F(x)) \geq R\}$ and $x_0 \leq \overline{x}_0 = \inf \{x: x(1-F(x)) \geq R\}$.
\label{dfn:thresholded_beta}
\end{theorem}
The proof is in Appendix \ref{ssec:best_quasi_regular_response}.
\iffalse
\begin{remark}
The thresholding strategy introduced in Definition \ref{definition_thresholded_strategies} is a special case of $\dtbeta$ in the case when $x_0 = 0$ and we will denote it $\tbeta$ for simplicity. As we will see in Section \ref{sec:optimal_strategies}, when $\alpha$ is small enough (but not 0 yet), $x_0 = 0$ is optimal. It thus makes sense to study both these strategies.
\end{remark}
\fi
\iffalse
This class of strategies solves the main drawback of the best response from \cite{tang2016manipulate}. If the value distribution $F_i$ is quasi-regular, then the bid distribution $F_{B}$ is also quasi-regular, offering a quasi-concave maximization problem (thus ``predictable" for the buyer) to the seller.
Figure \ref{fig:optimal_revenues} illustrates the different strategies as well as the corresponding optimization problems and the virtual values associated to the push-forward bid distributions. Understanding the strategic answer of the bidders helps avoiding worst-case scenario reasoning when studying the revenue of the sellers against strategic bidders. We now quantify precisely how the welfare is shared between strategic bidders and seller.
\fi


%The literature have only considered so far the 
%possible bidding strategies: 
%\begin{definition}[Thresholded bidding strategies]\cite{tang2016manipulate,nedelec2018thresholding}
%\label{dfn:thresholded_beta}
% A bidding strategy $\beta$ is called a thresholded bidding strategy if and only if there exists $r>0$ such that for all $x < r, h_{\beta}(x) = \psi_B(\beta(x)) = 0$. This family of functions can be parametrized with
%\begin{equation*}
%\beta_r^\gamma(x)=\frac{\gamma(r)(1-F(r))}{1-F(x)}\indicator{x< r}+\gamma(x)\indicator{x\geq r}\;,
%\end{equation*}
%with $r \in \mathbb{R}$ and $\gamma: \mathbb{R} \rightarrow \mathbb{R}$ strictly increasing.
%\end{definition}
%
%This class of continuous bidding strategies has two degrees of freedom : the threshold $r$ such that for all $x < r, h_{\beta}(x) = 0$ and the strategy $\gamma$ used beyond the threshold. We do not restrict the class of functions of $\gamma$ that can be used beyond the threshold. All the strategies defined in this class have the property to have a reserve value equal to zero, i.e. their reserve price is equal to their minimum bid, when the seller is welfare benevolent and the virtual value of $\gamma$ is positive beyond $r$. We show that there exists an optimal threshold $r$ for the strategic bidder that depends on the competition and that the optimal strategy to use for $x > r$ is to be truthful. The next lemma computes this optimal thresholded strategy by deriving a variant of Lemma \ref{lemma:directDerivativeRevenueSecondPriceAuction} in the class of thresholded strategies.
%
%thresholded strategies with a dirac \cite{tang2016manipulate}
%
%
%neural networks to learn the best response \cite{nedelec2019learning}
\iffalse
\section{Welfare sharing between seller and buyers}\label{sec:welfareSharing}

\fi
This section presents how the welfare is shared in the two-stage process with strategic bidders. 
\iffalse
First, we show how to numerically compute the best response and illustrate the variation of utility and payment with $\alpha$. After remarking and showing that the \emph{thresholded} strategy \cite{nedelec2018thresholding} is optimal for greater values of $\alpha$ than 0, we focus on this strategy and show the existence of a Nash equilibrium. It proves that even in the case of multiple strategic bidders, there exists strategies that enable bidders to take advantage of the learning stage of the seller.
\fi
\subsubsection{Welfare sharing with best quasi-regular response}
\begin{figure}[tbp]
  \centering
    \includegraphics[width=0.32\textwidth]{figures/welfare_no_reserve_1_with_sum_thomas_utility.pdf}
     \includegraphics[width=0.32\textwidth]{figures/welfare_no_reserve_1_with_sum_thomas_payment.pdf}
  \includegraphics[width=0.32\textwidth]{figures/optimal_thresholds_no_reserve.pdf}
  \caption{Welfare sharing with random reserve in stage 1: Left -- Utility of strategic bidder in the two-stage game as a function of $\alpha$. Middle -- Payment of strategic bidder in the two-stage game as a function of $\alpha$. The dotted lines corresponds to phase 1, the dashed ones to phase 2 and the plain line for the full game. The blue color is used for the bidder's utility and the red for her payment. The black color is used for the baseline of truthful bidding. Right: evolution of $x_0^*, x_1^*$ with $\alpha$.}
  \label{fig:welfare_vs_alpha}
\end{figure}
\label{sec:optimal_strategies}
We first show how to obtain numerically the best response $\dtbeta$ by solving the maximization problem of $U_\alpha$ restricted to the class of strategies described in Th. \ref{dfn:thresholded_beta}. This allows us to show how the bidder's utility and payment vary with $\alpha$.
\begin{theorem}
Given a two-stage process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$, the best response is of the form of $\tilde{\beta}_{x_0^*, x_1^*}$ and the utility $U_\alpha(\dtbeta)$ has the following derivatives:
\begin{align}
    \frac{\partial U_\alpha(\dtbeta\!)}{\partial x_0} \!=\! \alpha(1-F(x_0))G(x_0)H(x_0)
    -
    x_0 f(x_0) G_\alpha\!\!\left(\frac{x_1(1-F(x_1))}{(1-F(x_0))}\right)~~~~~~~~~~~\\
    \frac{\partial U_\alpha(\dtbeta\!)}{\partial x_1} 
    \!= \!
    f(x_1)\psi(x_1)
    \!\left(\!G_\alpha(x_1) - \lE_X\!\!\left(\!\indicator{x_0 \leq X \leq x_1}\frac{X}{(1-F(X))}g_\alpha\!\!\left(\!\frac{x_1(1-F(x_1))}{(1-F(X))}\!\right)\!\!\right)\!\!\right)
\end{align}
where $G_\alpha(x) = \alpha G(x)H(x) + (1-\alpha)G(x)$ and $\psi(x)=x-\frac{1-F(x)}{f(x)}$.
\label{thm:double_thresholded_derivatives}
\end{theorem}
The proof is in Appendix \ref{ssec:welfare_sharing_best_response}. We now use these results to compute numerically the best response in the following two-stage process: $P_1 = (G\!=\!U_{[0,1]}, H\!=\!0, r^*_{\tilde{\beta}_{x_0^*, x_1^*}}, F\!=\!U_{[0,1]})$ (uniformly distributed reserve in  stage 1)
   
\iffalse  
$P_2 = (G\!=\!U_{[0,1]}, H\!=\!1, r^*_{\tilde{\beta}_{x_0^*, x_1^*}}\!, F\!=\!U_{[0,1]})$ (no reserve in stage 1).
\fi

The results are presented in Fig. \ref{fig:welfare_vs_alpha}.
First, we recover the results from the literature corresponding to the extremes values of $\alpha$. For $\alpha = 1^-$, the payment and utility in the second stage are the ones of a 2$^\text{nd}$-price with monopoly price of value distribution. As $\alpha$ decreases, the total payment over the two stages quickly decreases (and utility increases) towards values that are even more favorable to the bidder than the ones of a 2$^\text{nd}$-price with no reserve price. 
\iffalse
This is consistent with the observations from \cite{nedelec2018thresholding} (case $\alpha=0$): if only one bidder is strategic, the payment of this strategic bidder can decrease even further than the one of a 2$^\text{nd}$-price with no reserve price. 
In Appendix \ref{ssec:plot_with_random_reserve}, we provide the same study with random reserve and show that the presence of exploration of the reserve prices in the first period (difference between left and right) does not impact much the payment/utility of the second period. It slightly decreases the advantage of the bidder, but not significantly.
\fi
Finally, we observe two regimes for $x_0^*$ (Fig. \ref{fig:welfare_vs_alpha}, right): for $\alpha < 0.8$ it is 0 and for $\alpha > 0.8$ it is the value that saturates the inequality constraint described by Th. \ref{dfn:thresholded_beta} between $x_0$ and $x_1$. This illustrates why we cannot only use first-order optimality condition: the optimal value is often reached on the edge of the feasible domain. We formalize this latter observation and shows that when $\alpha$ is small enough, the reserve value $x_0^*$ is exactly 0.
\begin{lemma}
Given a two-step process $(G, H, r_{\beta}^*, F)$ with $r^*_\beta = \inf \argmax_r R_B(r)$. If $\exists y \in [0,b], \forall x<y, \frac{G(x)H(x)}{f(x)} < x$ and $\frac{G(x)H(x)}{f(x)}$ is bounded on $[0,x^*]$ with $x^*=\inf\argmax_x R_X(x)$, then $\exists \alpha_0 > 0$ such that $\forall \alpha < \alpha_0$, 
\begin{align*}
(x^*_0,x^*_1) \in \argmax_{x_0, x_1}U_\alpha(\dtbeta) 
~~~ \Rightarrow ~~~ 
x_0^* = 0
\end{align*}
\label{thm:x0_to_0}
\end{lemma}
\vspace{-1em}
The proof can be found in Appendix \ref{ssec:welfare_sharing_best_response}.  $\frac{G(x)H(x)}{f(x)}$ being bounded on $[0,x^*]$ is satisfied if $F$ is MHR (monotonous hazard rate). $\frac{G(x)H(x)}{f(x)}<x$ is the key assumption. Intuitively, it can be interpreted as \emph{"if the bidder has enough mass under the competition, she can overbid at almost no cost on small values to decrease the reserve value to 0."}
This theorem shows that the \emph{thresholding} strategies are actually optimal for $\alpha$ small enough and not just for $\alpha = 0$.



\iffalse
 In the following subsections, we carry out a formal analysis for such strategies $\tilde{\beta}_{0, x_1} = \tilde{\beta}_{x_1}$ as we can more easily characterize the best response and prove Nash equilibria.
\subsection{Phase transition for the classical thresholding strategies in the two-stage game} 
\label{subsec:PhaseTransitionThresholding}
We suppose in this subsection that the seller commits to thresholding, i.e. $x_0=0$ with the notation above. The seller uses monopoly reserves in the second phase. 
%We have the following theorem. 
\begin{theorem}\label{thm:TwoStepProcessCommitment}
We call ${\mathcal G}_\alpha=\alpha G_1+(1-\alpha) G_2$, $G_1$ and $G_2$ being the distributions of the competition faced by the bidder in the two phases, possibly including reserve prices. We assume $\psi^{-1}(0)>0$.
If the buyer uses the thresholding strategy $\tbeta$ of Theorem \ref{dfn:thresholded_beta}  and commits to it, we have for their utility, if the seller is welfare benevolent~:
the utility has (in general) a discontinuity at $x_1=\psi^{-1}(0)$. For $x_1<\psi^{-1}(0)$, we have $U(0)\geq U(x_1)$. For $x_1>\psi^{-1}(0)$, the first order condition are the same as in \cite{nedelec2018thresholding,tang2016manipulate} where the distribution of the competition is now ${\mathcal G}_\alpha=\alpha G_1+(1-\alpha) G_2$. Call $x_1^*(\alpha)$ the unique solution of this problem. Hence, the optimal threshold is $\argmax_{x_1\in \{0,x_1^*(\alpha)\}} U(x_1)$. An optimal threshold at $x_1=0$ corresponds to bidding truthfully. 

\end{theorem}

\begin{lemma}[Phase transition in $\alpha$]\label{lemma:phaseTransition}
Assume the setup of Theorem \ref{thm:TwoStepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases and there is no reserve price in the first phase.  Then there is a critical value $\alpha_c$ for which, if $\alpha<\alpha_c$, it is preferable for the bidder to threshold and if $\alpha>\alpha_c$, it is preferable for the bidder to bid truthfully. 	
\end{lemma}
The proofs of the theorem and the lemma can be found in Section \ref{sec:ProofsSec3Thresholding} and we provide more details on the utility there. 
A graphical illustration of these results can be found in the Appendix, Figure \ref{fig:2StageNoReservesCommitment}.
\fi

